Causal effect of regulated Bitcoin futures on volatility and volume

In December 2017, two leading derivative exchanges, CBOE and CME, introduced the first regulated Bitcoin futures. Our aim is estimating their causal impact on Bitcoin volatility and trading volume. Employing a new causal approach, C-ARIMA, we find that the CME future triggered an increase in both outcomes. There is also evidence of a positive volume-volatility relationship and that the effect on volatility was partially due to the higher trading volumes induced by the launch of the contract. After controlling for the effect on volumes, we find that the CME instrument caused Bitcoin volatility to increase by more than double.

==> Tables/corr.tex <==

\centering
\begin{tabular}{rrrrrrrrrrrrrrrrrrr}
  \hline
 & y & eurusd\_vol & mxef\_vol & shc\_vol & inflation & eu.infl & eurusd & mxwo & mxef & shc & m1 & gdp & midrate & hash & eu.m1 & eu.gdp & ch.m1 & btcsupply \\ 
  \hline
y & 1.000 & 0.011 & -0.045 & -0.124 & 0.062 & 0.048 & 0.011 & -0.042 & -0.001 & -0.019 & 0.004 & 0.010 & 0.014 & 0.032 & 0.010 & -0.013 & -0.009 & 0.034 \\ 
  eurusd\_vol & -0.008 & 1.000 & 0.379 & 0.285 & -0.071 & 0.032 & 0.004 & -0.048 & -0.071 & -0.030 & -0.013 & -0.023 & 0.055 & 0.002 & -0.024 & -0.027 & 0.007 & -0.050 \\ 
  mxef\_vol & -0.056 & 0.331 & 1.000 & 0.349 & -0.031 & -0.003 & 0.007 & -0.093 & -0.127 & -0.096 & 0.001 & -0.088 & 0.051 & -0.031 & -0.070 & -0.103 & 0.006 & -0.015 \\ 
  shc\_vol & -0.138 & 0.273 & 0.369 & 1.000 & -0.174 & -0.102 & -0.027 & -0.059 & -0.102 & -0.123 & 0.014 & -0.041 & -0.026 & -0.006 & 0.021 & -0.036 & 0.019 & 0.035 \\ 
  inflation & 0.075 & 0.001 & -0.054 & -0.156 & 1.000 & 0.641 & 0.023 & -0.021 & -0.021 & -0.035 & -0.036 & 0.010 & 0.002 & -0.005 & -0.051 & -0.003 & -0.044 & -0.000 \\ 
  eu.infl & 0.101 & 0.089 & -0.012 & -0.104 & 0.589 & 1.000 & 0.011 & 0.000 & -0.006 & 0.008 & -0.011 & 0.006 & -0.018 & -0.001 & -0.031 & 0.006 & -0.049 & 0.002 \\ 
  eurusd & 0.022 & -0.011 & 0.011 & -0.014 & 0.014 & 0.021 & 1.000 & 0.032 & 0.032 & -0.062 & -0.005 & -0.053 & 0.006 & -0.015 & -0.023 & -0.072 & 0.052 & 0.022 \\ 
  mxwo & 0.004 & -0.019 & -0.047 & -0.029 & 0.033 & 0.025 & 0.063 & 1.000 & 0.637 & 0.213 & -0.018 & -0.003 & 0.035 & -0.039 & -0.020 & -0.023 & 0.018 & -0.010 \\ 
  mxef & 0.026 & -0.049 & -0.089 & -0.089 & 0.027 & 0.027 & 0.043 & 0.596 & 1.000 & 0.411 & -0.003 & 0.010 & 0.039 & -0.012 & -0.013 & 0.013 & -0.012 & -0.023 \\ 
  shc & -0.028 & -0.002 & -0.037 & -0.022 & -0.038 & -0.003 & -0.017 & 0.181 & 0.365 & 1.000 & -0.011 & 0.019 & -0.005 & -0.027 & 0.013 & 0.011 & -0.024 & 0.004 \\ 
  m1 & -0.020 & -0.005 & 0.010 & 0.024 & -0.018 & -0.005 & 0.018 & -0.031 & -0.010 & -0.010 & 1.000 & -0.042 & -0.004 & -0.014 & 0.067 & -0.045 & 0.058 & 0.087 \\ 
  gdp & -0.000 & -0.010 & -0.078 & -0.056 & -0.008 & -0.006 & -0.072 & -0.024 & 0.013 & 0.004 & -0.037 & 1.000 & -0.007 & -0.014 & 0.403 & 0.827 & -0.014 & 0.023 \\ 
  midrate & 0.032 & 0.038 & 0.047 & -0.038 & -0.006 & -0.007 & 0.035 & -0.014 & 0.032 & -0.026 & -0.005 & -0.010 & 1.000 & -0.047 & -0.012 & -0.007 & 0.000 & -0.005 \\ 
  hash & 0.039 & 0.006 & -0.020 & -0.017 & -0.002 & 0.002 & -0.009 & -0.045 & -0.019 & -0.032 & -0.035 & -0.024 & -0.016 & 1.000 & -0.031 & -0.014 & -0.022 & 0.103 \\ 
  eu.m1 & 0.033 & -0.017 & -0.067 & -0.010 & -0.006 & 0.002 & -0.034 & -0.025 & -0.008 & -0.011 & 0.048 & 0.557 & -0.018 & -0.039 & 1.000 & 0.452 & 0.090 & 0.107 \\ 
  eu.gdp & -0.001 & -0.010 & -0.079 & -0.056 & -0.008 & -0.006 & -0.072 & -0.024 & 0.013 & 0.004 & -0.038 & 1.000 & -0.010 & -0.024 & 0.557 & 1.000 & -0.091 & -0.001 \\ 
  ch.m1 & -0.011 & 0.016 & 0.043 & 0.059 & 0.003 & -0.035 & 0.059 & 0.019 & 0.028 & -0.030 & 0.012 & -0.121 & 0.002 & -0.005 & -0.137 & -0.124 & 1.000 & 0.061 \\ 
  btcsupply & 0.035 & -0.048 & -0.016 & 0.053 & -0.001 & 0.001 & 0.034 & -0.015 & -0.026 & -0.001 & 0.091 & 0.023 & -0.011 & 0.373 & 0.078 & 0.022 & 0.061 & 1.000 \\ 
   \hline
\end{tabular}

